A coordination-free, convergent, and safe replicated tree

The tree is an essential data structure in many applications. In a distributed application, such as a distributed file system, the tree is replicated.To improve performance and availability, different clients should be able to update their replicas concurrently and without coordination. Such concurrent updates converge if the effects commute, but nonetheless, concurrent moves can lead to incorrect states and even data loss. Such a severe issue cannot be ignored; ultimately, only one of the conflicting moves may be allowed to take effect. However, as it is rare, a solution should be lightweight. Previous approaches would require preventative cross-replica coordination, or totally order move operations after-the-fact, requiring roll-back and compensation operations. In this paper, we present a novel replicated tree that supports coordination-free concurrent atomic moves, and provably maintains the tree invariant. Our analysis identifies cases where concurrent moves are inherently safe, and we devise a lightweight, coordination-free, rollback-free algorithm for the remaining cases, such that a maximal safe subset of moves takes effect. We present a detailed analysis of the concurrency issues with trees, justifying our replicated tree data structure. We provide mechanized proof that the data structure is convergent and maintains the tree invariant. Finally, we compare the response time and availability of our design against the literature.

==> sections/proofs.tex <==
\section{Proofs}
\label{sec:proofs}
Section for describing the formal semantics of the proof and documenting proof tactics.


==> sections/seqspec.tex <==
Initial State: $Nodes = \{(root \rightarrow \emptyset)\}$\\
Invariant: $\forall n. n \in Nodes \implies reachable(n)$\\
Operations:\\
$\{Pre_{add}: root \rightarrow^* p$ \tab \dots \dots \textcolor{blue}{p is reachable from root} \\
\tab $\wedge n \notin Nodes\}$ \tab \dots \dots \textcolor{blue}{n is not already present in the tree}\\
$add(n, p): Nodes \cup \{(n \rightarrow p)\}$\\

$\{Pre_{remove}: root \rightarrow^* n$ \tab \dots \dots \textcolor{blue}{n is reachable from the root} \\
\tab \tab $\wedge \nexists n'. n \rightarrow^* n'\}$ \tab \dots \dots \textcolor{blue}{n is a leaf node}\\
$remove(n, p): Nodes \setminus \{(n \rightarrow p)\}$\\

$\{Pre_{move}: root \rightarrow^* p$ \tab \dots \dots \textcolor{blue}{p is reachable from the root} \\
\tab $\wedge root \rightarrow^* p'$ \tab \dots \dots \textcolor{blue}{p' is reachable from the root} \\
\tab $\wedge p \rightarrow n$ \tab \dots \dots \textcolor{blue}{p is  the parent of c} \\
\tab $\wedge \neg(c \rightarrow^* p')\}$ \tab \dots \dots \textcolor{blue}{c is not an ancestor of p'}\\
$move(n, p, p'): Nodes \setminus \{(n \rightarrow p)\} \wedge Nodes \cup \{(n \rightarrow p')\}$\\
